Qalam : A Multimodal LLM for Arabic Optical Character and Handwriting Recognition

Arabic Optical Character Recognition (OCR) and Handwriting Recognition (HWR) pose unique challenges due to the cursive and context-sensitive nature of the Arabic script. This study introduces Qalam, a novel foundation model designed for Arabic OCR and HWR, built on a SwinV2 encoder and RoBERTa decoder architecture. Our model significantly outperforms existing methods, achieving a Word Error Rate (WER) of just 0.80% in HWR tasks and 1.18% in OCR tasks. We train Qalam on a diverse dataset, including over 4.5 million images from Arabic manuscripts and a synthetic dataset comprising 60k image-text pairs. Notably, Qalam demonstrates exceptional handling of Arabic diacritics, a critical feature in Arabic scripts. Furthermore, it shows a remarkable ability to process high-resolution inputs, addressing a common limitation in current OCR systems. These advancements underscore Qalam's potential as a leading solution for Arabic script recognition, offering a significant leap in accuracy and efficiency.

==> decoder.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrr}\toprule
\textbf{Dataset Type} &\textbf{Line Based} &\textbf{Word Based} &\textbf{Character Based} &\textbf{Average} \\\midrule
\textbf{Roberta} &64.13 &11.11 &13.26 &29.50 \\
\textbf{XLM-roberta} &43.22 &6.39 &4.74 &18.12 \\
\textbf{ARBERT} &35.91 &2.39 &0.94 &\textbf{13.08} \\
\textbf{MARBERT} &49.28 &7.28 &7.32 &21.29 \\
\textbf{MARBERTv2} &38.58 &5.16 &2.48 &15.40 \\
\bottomrule
\end{tabular}}
\caption{Decoder Selection with DeIT as constant encoder}\label{tab: }
\end{table*}

==> encoder.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrr}\toprule
\textbf{Dataset Type} &\textbf{Line Based} &\textbf{Word Based} &\textbf{Character Based} &\textbf{Average} \\\midrule
\textbf{DeiT} &43.22 &6.39 &4.74 &\textbf{18.12} \\
\textbf{BeiT} &47.62 &9.31 &6.40 &21.11 \\
\textbf{ViT} &56.70 &9.36 &7.24 &24.43 \\
\textbf{Swin} &52.36 &7.96 &7.62 &22.65 \\
\bottomrule
\end{tabular}}
\caption{Encoder Selection with XLMR as constant decoder}\label{tab: }
\end{table}

==> final.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrr}\toprule
\textbf{Models/Datasets} & \textbf{Line Based} & \textbf{Word Based} & \textbf{Character Based} \\\midrule
Tesseract $\downarrow$ & $53.67$ & $97.27$ & $116.53$ \\
TrOCR $\downarrow$ & $45.85$ & $4.33$ & $12.80$ \\
SOTA $\downarrow$ & $12.24$ & $4.42$ & $1.08$ \\
ArOCR $\downarrow$ & $\textbf{4.12}$ & $\textbf{0.15}$ & $\textbf{0.03}$ \\
\bottomrule
\end{tabular}}
\caption{Final Results}\label{tab: }
\end{table*}


==> limitations.tex <==
\section{Limitations}


==> methodolgy.tex <==
\section{Methodology} \label{methodology}

The Vision Encoder-Decoder architecture amalgamates the original Transformer with the Vision Transformer (ViT) by retaining the encoder-decoder structure while modifying the encoder to accept images divided into 16x16 pixel patches. During training, the decoder is provided with the ground-truth caption as input through a process known as teacher forcing, and the encoder's hidden states serve as inputs for the cross-attention layers. The model has trained autoregressively for the next token prediction, utilizing causal (or unidirectional) self-attention, ensuring that a given token can only attend to preceding tokens.

To implement this architecture, we employed the Vision Encoder Decoder class from the Hugging Face Transformers library. We experimented with multiple Vision Transformers for the encoder while leveraging pre-trained weights from the BERT-based auto-encoding Transformers for the decoder.

In this paper, we present our findings on applying the Vision Encoder-Decoder architecture for Arabic OCR, demonstrating its effectiveness in addressing the challenges specific to Arabic handwriting recognition. By employing this advanced methodology, we seek to contribute to the ongoing research in the field, ultimately improving the performance and accuracy of Arabic OCR systems.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figs/arch.pdf}
  \caption{Diagram from PDF}
  \label{fig:diagram}
\end{figure}

==> vision.tex <==
\subsection{Vision Transformers: Overview}


